Evolve Smoothly, Fit Consistently: Learning Smooth Latent Dynamics For Advection-Dominated Systems

We present a data-driven, space-time continuous framework to learn surrogate models for complex physical systems described by advection-dominated partial differential equations. Those systems have slow-decaying Kolmogorov n-width that hinders standard methods, including reduced order modeling, from producing high-fidelity simulations at low cost. In this work, we construct hypernetwork-based latent dynamical models directly on the parameter space of a compact representation network. We leverage the expressive power of the network and a specially designed consistency-inducing regularization to obtain latent trajectories that are both low-dimensional and smooth. These properties render our surrogate models highly efficient at inference time. We show the efficacy of our framework by learning models that generate accurate multi-step rollout predictions at much faster inference speed compared to competitors, for several challenging examples.

==> background.tex <==

\section{Background}
\label{sec:backgroud}


\begin{figure}[t]
% \begin{center}
%\framebox[4.0in]{$\;$}

\centering
\includegraphics[width=0.75\textwidth]{iclr2023/figures/diagram_dyn_weights.png}
% \end{center}
\caption{Diagram of the evolution in latent space.}\label{fig:diagram}
\end{figure}

